On the Importance of Sampling in Training GCNs: Tighter Analysis and Variance Reduction

Graph Convolutional Networks (GCNs) have achieved impressive empirical advancement across a wide variety of semi-supervised node classification tasks. Despite their great success, training GCNs on large graphs suffers from computational and memory issues. A potential path to circumvent these obstacles is sampling-based methods, where at each layer a subset of nodes is sampled. Although recent studies have empirically demonstrated the effectiveness of sampling-based methods, these works lack theoretical convergence guarantees under realistic settings and cannot fully leverage the information of evolving parameters during optimization. In this paper, we describe and analyze a general doubly variance reduction schema that can accelerate any sampling method under the memory budget. The motivating impetus for the proposed schema is a careful analysis of the variance of sampling methods where it is shown that the induced variance can be decomposed into node embedding approximation variance (zeroth-order variance) during forward propagation and layerwise-gradient variance (first-order variance) during backward propagation. We theoretically analyze the convergence of the proposed schema and show that it enjoys an $\mathcal{O}(1/T)$ convergence rate. We complement our theoretical results by integrating the proposed schema in different sampling methods and applying them to different large real-world graphs.

==> previous_comments.tex <==
\clearpage
\noindent\textbf{NeurIPS21 review}
\begin{itemize}
    \item Reduce the induced variance during training will not guarantee to have better generalization results on the test set. Discuss the connection between variance reduction and the generalization aspect. \weilin{should we discuss generalization?}
    \item Experiment on new sampling strategies + model architecture. \weilin{too many work to do and the payback is too less}
    \item The dataset used in this paper are small-scale datasets. I believe for some small datasets, we can easily train in a full-batch manner on GPU. I am not convinced that the proposed algorithm is scalable to large graphs due to Full-batch gradient. \mr{}
    \item The baseline results reported in the paper don't match the result shown in the prior work (such as results reported in GraphSAINT are much higher than in this paper). \weilin{we already discuss}
    \item In the SGCN+ section, the authors should have a proper discussion on the differences between SGCN+ and VRGCN. The proposed "snapshot + regular step" update rules seem exactly the same as the historical utilization steps of VRGCN. \weilin{we already discuss}
    \item The conclusion from Theorem 1 is wrong. To conclude that "the gradient norm of SGCN ... suffers from a constant residual error  that is not decreasing as the number of iterations T increases", we need a lower bound. However, Theorem 1 shows an upper bound. \mr{}
    \item Assumption 3 is too strong. The F-norm of the Laplacian grows with the graph size. Requiring  to be bounded implies the algorithm is not scalable with respect to the graph size. \weilin{we cannot do anything} \mr{refer to other papers that made same assumptions}
    \item matrix P is not defined clearly. From the main text, the description is very confusing that  is "defined as the column-wise expectation of the sparser Laplacian matrices". What does column-wise expectation mean? What is "sparser"? \weilin{we have discussion in appendix}
    \item Mostly importantly, the equations of 85 and 86 are wrong. Here we are calculating expectation. Can you explain why we can ignore all the non-linearities like multiplication and  to place expectation on each individual quantity? \weilin{we didnt}
    \item SGD + Adam. refer to that paper, sgd is too slow.
\end{itemize}

\noindent\textbf{ICML21 review}
\begin{itemize}
    \item Issue 1: One of the reviewers points out some issues in the proof the Theorem 3. More specifically, when employing variance reduction algorithms, due to the recursive update rule, the norm of hidden features cannot be bounded as the algorithm without using a variance reduction. \weilin{We resolve issue 1 by adding an early stop criterion in the algorithm and update the proof accordingly. Notice that this early stopping criterion is not just used for theoretical analysis, it also exists in our implementation.}
    \item Issue 2: One of the reviewers points out there exists a typo in the caption. \weilin{We resolve issue 2 by updating the figure in the supplementary.}
    \item Issue 3: Reviewers recommend we add standard deviation and wall clock in the reported F1-score results. \weilin{We resolve issue 3 by reporting the standard deviation in Table 1 and report convergence w.r.t. wall-clock time in the supplementary.}
    \item  Issue 4: One of the reviewers is wondering how the residual error issue is resolved in the SGCN+.
\end{itemize}

\noindent\textbf{ICLR21 review (most points already appears before)}
\begin{itemize}
    \item A minor point: The paper says “the data points in these works are sampled independently, but the data points (nodes) in SGCN are sampled node- or layer-dependent according to the graph structure.” The data samples in compositional optimization do not need to be independent. The only requirement is that the stochastic function with the data samples is unbiased
    \item Adam vs SGD \mr{refer to VRGCN papers}
\end{itemize}

\mr{Read the call and add some keywords to the abstract and intro according to CFP}

==> section/experiment_configs.tex <==
\begin{table}[h]
\vspace{-3mm}
\caption{Configuration of different sampling algorithms during training}
\label{table:train_config}
\centering
\scalebox{0.92}{
\begin{tabular}{lcccccc}
\toprule
                                 & \texttt{GraphSAGE} & \texttt{VRGCN} & \texttt{Exact} & \texttt{FastGCN} & \texttt{LADIES} & \texttt{GraphSAINT} \\ \midrule
\textbf{Mini-batch size}         & 512                & 512            & 512            & 512             & 512             & 2048                \\
\textbf{Sampled neighbors}       & 5                  & 2              & All            & -                & -               & -                   \\ 
\textbf{Samples in layerwise}    & -                  & -              & -              & 4096             & 512             & 2048                \\ \bottomrule
\end{tabular}}
\end{table}

==> section/experiment_details.tex <==
\section{Experiment configurations}\label{section:exp-config}

\paragraph{Hardware specification and environment}.~
We run our experiments on a single machine with Intel i5-7500, NVIDIA GTX1080 GPU (8GB memory) and, 32GB RAM memory. 
The code is written in Python 3.7 and we use PyTorch 1.4 on CUDA 10.1 to train the model on GPU. 
During each epoch, we randomly construct 10 mini-batches in parallel. 

\paragraph{Implementation details.}~
To demonstrate the effectiveness of doubly variance reduction, we modified the PyTorch implementation of {GCN}~\citep{semigcn}\footnote{\url{https://github.com/tkipf/pygcn}} to add \texttt{LADIES}~\citep{ladies}, \texttt{FastGCN}~\citep{fastgcn}, \texttt{GraphSAGE}~\citep{graphsage}, \texttt{GraphSAINT}~\citep{graphsaint}, \texttt{VRGCN}~\citep{control_variacne_gcn}, and \texttt{Exact} sampling mechanism. 
Then, we implement \texttt{SGCN+} and \texttt{SGCN++} on the top of each sampling method to illustrate how zeroth-order variance reduction and doubly variance reduction help for GCN training. 
The source code for our experiments is available on \href{https://anonymous.4open.science/r/68b416be-b4c8-432c-b2c8-604fa339f81f/}{https://anonymous.4open.science/r/68b416be-b4c8-432c-b2c8-604fa339f81f/}.

By default, we train $2$-layer GCNs with hidden state dimension of $256$, element-wise ELU as the activation function and symmetric normalized Laplacian matrix $\mathbf{L} = \mathbf{D}^{-1/2} \mathbf{A} \mathbf{D}^{-1/2}$. 
We use \emph{mean-aggregation} for single-class classification task and \emph{concatenate-aggregation} for multi-class classification.
% The detailed graph convolutional network structure is defined as
% \begin{equation*}
%     \begin{aligned}
%     & \texttt{ELU}(\texttt{GraphConvolution}(\texttt{nfeat}, \texttt{nhid}=256)) \\
%     & \texttt{ELU}(\texttt{GraphConvolution}(\texttt{nhid}=256, \texttt{nhid}=256)) \\
%     & \texttt{Linear}(\texttt{nhid}=256, \texttt{nclasses})
%     \end{aligned}
% \end{equation*}
The default mini-batch batch size and sampled node size are summarized in Table~\ref{table:train_config}.
We update the model using Adam optimizer with a learning rate of $0.01$. 
For \texttt{SGCN++}, historical node embeddings are first calculated on GPUs and transfer to CPU memory using PyTorch command \texttt{Tensor.to(device)}. 
Therefore, no extra GPU memory is required when training with \texttt{SGCN++}. 
To balance the staleness of snapshot model and the computational efficiency, as default we choose snapshot gap $K=10$ and early stop inner-loop if the Euclidean distance between current step gradient to snapshot gradient is larger than $0.002$ times the norm of snapshot gradient.

\input{sections/ex}

During training, for each epoch we construct $10$ mini-batches in parallel using Python package \texttt{multiprocessing} and perform training on the sampled $10$ mini-batches. 
To achieves a fair comparison of different sampling strategies in terms of sampling complexity, we implement all sampling algorithms using \texttt{numpy.random} and \texttt{scipy.sparse} package. 

We have to emphasize that, in order to better observe the impact of sampling on convergence, we have not use any augmentation methods (e.g., ``layer normalization'', ``skip-connection'', and ``attention''), which have been proven to impact the GCN performance in~\cite{cai2020graphnorm,dwivedi2020benchmarkgnns}.
Notice that we are not criticizing the usage of these augmentations. 
Instead, we use the most primitive network structure to better explore the impact of sampling and variance reduction on convergence.

\note{
\paragraph{Comparison of SGD and Adam.}
It is worth noting that Adam optimizer is used as the default optimizer during training. We choose Adam optimizer over SGD optimizer for the following reasons: 
\begin{itemize}
    \item [(a)] Baseline methods training with SGD cannot converge when using a constant learning rate due to the bias and variance in stochastic gradient (Adam has some implicit variance reduction effect, which can alleviate the issue). 
    The empirical result of SGD trained baseline models has a huge performance gap to the one trained with Adam, which makes the comparison meaningless. 
    For example in Figure~\ref{fig:sgd_vs_adam_ppi}, we compare Adam and SGD optimizer on PPI dataset. For Adam optimizer we use PyTorch's default learning rate $0.01$, and for SGD optimizer we choose learning rate as $0.1$, which is selected as the most stable learning rate from range $[0.01, 1]$ for this dataset. Although the SGD is using a learning rate $10$ times larger than Adam, it requires $100$ times more iterations than Adam to reach the early stop point (valid loss do not decrease for $200$ iterations), and suffers a giant performance gap when comparing to Adam optimizer. 
    \item [(b)] Most public implementation of GCNs, including all implementations in PyTorch Geometric and DGL packages, use Adam optimizer instead of SGD optimizer.
    \item [(c)] In this paper, we mainly focus on how to estimate a stabilized stochastic gradient, instead of how to take the existing gradient for weight update. 
    We employ Adam optimizer for all algorithms during experiment, which lead to a fair comparison.
\end{itemize}
}

\begin{figure}
    \captionsetup{labelfont={color=DarkCyan}}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/sgd_vs_adam_ppi.pdf}
    \caption{\note{Comparison of doubly variance reduction and vanilla sampling-based GCN training on PPI dataset with SGD (learning rate $0.1$) and Adam optimizer (learning rate $0.01$). All other configurations are as default.}}
    \label{fig:sgd_vs_adam_ppi}
\end{figure}

\paragraph{Dataset statistics.}~
We summarize the dataset statistics in Table~\ref{table:datasets}.

\begin{table}[h]
\vspace{0mm}
\caption{Summary of dataset statistics. 
\textbf{m} stands for \textbf{m}ulti-class classification, and \textbf{s} stands for \textbf{s}ingle-class.
}
\label{table:datasets}
\centering
% \scalebox{1.0}{ %arxiv
\begin{tabular}{rcccccc}
\toprule
\textbf{Dataset}   & \textbf{Nodes} & \textbf{Edges} & \textbf{Degree} & \textbf{Feature} & \textbf{Classes} & \textbf{Train/Val/Test} \\ \midrule
% \textbf{Pubmed}    & 19,717         & 44,338         & 3               & 500              & 3(\textbf{s})          & 92\%/~3\%/~5\%          \\ \hline
\textbf{PPI}       & $14,755$         & $225,270$        & $15$              & $50$               & $121$(\textbf{m})          & $66\%/12\%/22\%$          \\ 
\textbf{PPI-Large} & $56,944$         & $818,716$        & $14$              & $50$               & $121$(\textbf{m})          & $79\%/11\%/10\%$          \\ 
\textbf{Flickr}    & $89,250$         & $899,756$        & $10$              & $500$              & $7$ (\textbf{s})               & $50\%/25\%/25\%$          \\ 
\textbf{Reddit}    & $232,965$        & $11,606,919$     & $50$              & $602$              & $41$(\textbf{s})               & $66\%/10\%/24\%$          \\ 
\textbf{Yelp}      & $716,847$        & $6,977,410$      & $10$              & $300$              & $100$(\textbf{m})          & $75\%/10\%/15\% $         \\ 
\bottomrule
% \textbf{Amazon}    & 1,598,960      & 132,169,734    & 83              & 200              & 107(\textbf{m})          & 85\%/5\%/10\%          \\ \hline
\end{tabular}
% }
\vskip -0.1in
\end{table}

